Understanding GEMM Performance and Energy on NVIDIA Ada Lovelace: A Machine Learning-Based Analytical Approach

Analytical framework for predicting General Matrix Multiplication (GEMM) performance on modern GPUs, focusing on runtime, power consumption, and energy efficiency. Our study employs two approaches: a custom-implemented tiled matrix multiplication kernel for fundamental analysis, and NVIDIA's CUTLASS library for comprehensive performance data collection across advanced configurations. Using the NVIDIA RTX 4070 as our experimental platform, we developed a Random Forest-based prediction model with multi-output regression capability. Through analysis of both naive tiled matrix multiplication with varying tile sizes (1 to 32) and 16,128 CUTLASS GEMM operations across diverse configurations, we identified critical performance patterns related to matrix dimensions, thread block configurations, and memory access patterns. Our framework achieved exceptional accuracy with an R^2 score of 0.98 for runtime prediction (mean error 15.57%) and 0.78 for power prediction (median error 5.42%). The system successfully predicts performance across matrix sizes, demonstrating robust scaling behavior. Our results show that optimal tile size selection can improve performance by up to 3.2x while reducing power consumption by 22% compared to baseline configurations. Analysis of shared memory utilization and SM occupancy reveals that tile sizes of 16x16 achieve the best balance between parallelism and resource usage. The implementation of our framework, including prediction models and analysis tools, is available as an open-source project at GPPerf [https://github.com/pavlyhalim/GPPerf].

==> references.tex <==
\begin{thebibliography}{13}

\bibitem{ali2023performance}
G.~Ali, M.~Side, S.~Bhalachandra, N.~J.~Wright, and Y.~Chen,
``Performance-aware energy-efficient {GPU} frequency selection using {DNN}-based models,''
in \emph{International Conference on Parallel Processing}.
ACM, 2023.

\bibitem{wang2024dso}
Q.~Wang et al.,
``{DSO}: A {GPU} energy efficiency optimizer by fusing dynamic and static information,''
\emph{arXiv preprint},
2024.

\bibitem{czarnul2019energy}
P.~Czarnul, J.~Proficz, and A.~Krzywaniak,
``Energy-aware high-performance computing: Survey of state-of-the-art tools, techniques, and environments,''
\emph{Wiley Online Library},
2019.

\bibitem{gpu_paper_2024}
Various,
``Energy-aware {GPU} performance prediction and optimization framework,''
NYU,
Tech. Rep.,
2024.

\bibitem{nvidia_docs}
{NVIDIA Corporation},
``{CUDA C++} programming guide,''
Version 12.2,
2023.

\bibitem{wang2018performance}
X.~Wang, K.~Huang, A.~Knoll, and X.~Qian,
``Performance prediction of {GPU}-based deep learning applications,''
in \emph{IEEE International Symposium on Performance Analysis of Systems and Software},
2018.

\bibitem{mei2013measurement}
X.~Mei, L.~S.~Yung, K.~Zhao, and X.~Chu,
``A measurement study of {GPU DVFS} on energy conservation,''
in \emph{HotPower},
2013.

\bibitem{guerreiro2020dvfs}
J.~Guerreiro, A.~Ilic, N.~Roma, and P.~Tom{\'a}s,
``{DVFS}-aware application classification to improve {GPGPUs} energy efficiency,''
\emph{Parallel Computing},
2020.

\bibitem{hong2009analytical}
S.~Hong and H.~Kim,
``An analytical model for a {GPU} architecture with memory-level and thread-level parallelism awareness,''
\emph{ACM SIGARCH Computer Architecture News},
vol.~37,
no.~3,
pp.~152--163,
2009.

\bibitem{braun2020simple}
L.~Braun, S.~Nikas, C.~Song, V.~Heuveline, and H.~Fr{\"o}ning,
``A simple model for portable and fast prediction of execution time and power consumption of {GPU} kernels,''
\emph{ACM Transactions on Architecture and Code Optimization},
vol.~17,
no.~4,
pp.~1--25,
2020.

\bibitem{nagasaka2010statistical}
H.~Nagasaka, N.~Maruyama, A.~Nukada, T.~Endo, and S.~Matsuoka,
``Statistical power modeling of {GPU} kernels using performance counters,''
in \emph{International Conference on Green Computing},
2010,
pp.~115--122.

\bibitem{boughzala2020predicting}
D.~Boughzala, L.~Lef{\`e}vre, and A.-C.~Orgerie,
``Predicting the energy consumption of {CUDA} kernels using {SimGrid},''
\emph{SBAC-PAD 2020},
pp.~191--198,
2020.

\bibitem{jammal2023preliminary}
F.~Jammal, N.~Aljabri, M.~Al-Hashimi, M.~Saleh, and O.~Abulnaja,
``A preliminary empirical study of the power efficiency of matrix multiplication,''
\emph{Electronics},
vol.~12,
no.~7,
p.~1599,
2023.

\end{thebibliography}
